MGCP: A Multi-Grained Correlation based Prediction Network for Multivariate Time Series

Multivariate time series prediction is widely used in daily life, which poses significant challenges due to the complex correlations that exist at multi-grained levels. Unfortunately, the majority of current time series prediction models fail to simultaneously learn the correlations of multivariate time series at multi-grained levels, resulting in suboptimal performance. To address this, we propose a Multi-Grained Correlations-based Prediction (MGCP) Network, which simultaneously considers the correlations at three granularity levels to enhance prediction performance. Specifically, MGCP utilizes Adaptive Fourier Neural Operators and Graph Convolutional Networks to learn the global spatiotemporal correlations and inter-series correlations, enabling the extraction of potential features from multivariate time series at fine-grained and medium-grained levels. Additionally, MGCP employs adversarial training with an attention mechanism-based predictor and conditional discriminator to optimize prediction results at coarse-grained level, ensuring high fidelity between the generated forecast results and the actual data distribution. Finally, we compare MGCP with several state-of-the-art time series prediction algorithms on real-world benchmark datasets, and our results demonstrate the generality and effectiveness of the proposed model.

==> algorithm/AFNO.tex <==
\begin{algorithm}[H]
\setstretch{1.12}
\caption{The Adaptive Fourier Neural Operators}
\KwIn{
 \ $X$   \\}
$bias = X$

$\Bar{X} = \text{RFFT2}(X)$

$\Bar{X}^{'} = \Bar{X}.\text{Reshape}(b, h, w//2+1, k, d/k)$

$\Tilde{X} = W_2\text{Relu}(W_1\Bar{X}^{'}+b_1)+b_2$

$\Tilde{X}^{'} = \Tilde{X}.\text{Reshape}(b, h, w//2+1, d)$

$\Tilde{X}^{''} = \text{SoftShrink}(\Tilde{X}^{'})$

$\hat{X} = \text{IRFFT2}(\Tilde{X}^{''})$

$\hat{X}^{'} = \hat{X}+ bias$
 
\KwOut{\ $\hat{X}^{'}$ \\ }
\label{alg:AFNO}
\end{algorithm}

==> algorithm/Decoder.tex <==
\begin{algorithm}[H]
\setstretch{1.12}
\caption{The Attention Decoder}
\KwIn{
 \  $X$, $E_f$   \\}
 $\overline{X}=\text{Position}(\text{Linear}(X))$
 
 $Q_1,K_1,V_1=\text{Linear}(\tilde{X})$
 
 \#self attention
 
 $Att_1=\text{softmax}\left( \frac{Q_1K^T_1}{\sqrt{d_k}}\right)V_1$

$Q_2=\text{Linear}(\text{LayerNorm}(Att_1))$

 $K_2,V_2=\text{Linear}(E_f)$ 
 
 \#cross attention
 
 $Att_2=\text{softmax}\left( \frac{Q_2K^T_2}{\sqrt{d_k}}\right)V_2$
  
 $\tilde{X}=\text{LayerNorm}(\text{Linear}(\text{LayerNorm}(Att_2)))$
 
\KwOut{\ $\tilde{X}$ \\ }
\label{alg:decoder}
\end{algorithm}

==> algorithm/Encoder.tex <==
\begin{algorithm}[H]
\setstretch{1.12}
\caption{The Attention Encoder}
\KwIn{
 \ $X$,   \\}
 $\overline{X}=\text{Position}(\text{Linear}(X))$
 
 $Q,K,V=\text{Linear}(\overline{X})$
 
 \#self attention
 
 $Att=softmax\left( \frac{QK^T}{\sqrt{d_k}}\right)V$
 
 $\tilde{X}=\text{LayerNorm}(\text{Linear}(\text{LayerNorm}(Att)))$
 
\KwOut{\ $\tilde{X}$ \\ }
\label{alg:encoder}
\end{algorithm}



==> algorithm/MGCP.tex <==
\begin{algorithm}[h]
\setstretch{1.3}
\caption{The Network Structure of The Multi-Grained Correlations-based Prediction Network.}
\label{alg:MGCP2}
\KwIn{historical values $X_{1:T}$, covariate features $V_{1:T+\tau}$, true future values $X_{T+1:T+\tau}$}
\smallskip
\hrule
\smallskip
\textbf{$\#$The Latent Space Mapper:}

$X_{1:T+\tau}^{'}=\text{Emb}(X_{1:T+\tau})$

$X_{1:T}^{''}= \text{AFNO}_1(X_{1:T}^{'})$

$X_{T+1:T+\tau}^{''}= [\text{AFNO}_2(X_{1:T+\tau}^{'})]_{T+1:T+\tau}$

$H^{(0)} =\text{MLP}(X_{1:T+\tau}^{''})$

$M = \text{GRU}(H_{1:T}^{(0)})$

$\tilde{A} = \text{softmax}\left(\frac{MW_1(MW_2)^T}{\sqrt{d_k}}\right)$

$A = \frac{1-\beta}{2}(\tilde{A}+\tilde{A}^T) + \beta I_N$ 

\For{$l \in {1, 2, \ldots, L}$}{
$H^{(l)} = \sigma\left(D^{-\frac{1}{2}}AD^{-\frac{1}{2}}H^{(l-1)}\right)$
}

$H = H^{(L)}$ 

\medskip
\hrule
\smallskip
\textbf{$\#$The Sequence Predictor:}

$E_f = \text{Encoder}(\text{Concat}(H_{1:T}, V_{1:T}))$

$\hat{H}_{T+1:T+\tau} = \text{Decoder}(V_{T+1:T+\tau},E_f)$

\medskip
\hrule
\smallskip
\textbf{$\#$The Restoration Component:}

$H_{1:T+\tau}^{'}=\text{Emb}(\text{Concat}(H_{1:T}, \hat{H}_{T+1:T+\tau}))$

$H_{1:T+\tau}^{''}= \text{AFNO}_3(X_{1:T}^{'};W_1^{'},W_2^{'})$


$\hat{X}_{T+1:T+\tau} =[\text{MLP}(X_{1:T+\tau}^{''})]_{T+1:T+\tau}$
\medskip
\hrule
\smallskip
\textbf{$\#$The Conditional Discriminator:}

$\Bar{A}=D^{-\frac{1}{2}} A D^{-\frac{1}{2}}$

$E_f^{'}=\text{Encoder}(\text{Concat}(\Bar{A}X_{1:T},V_{1:T})) $

$Y=\text{MLP}(\text{Decoder}(\text{Concat}(\Bar{A}X_{T+1:T+\tau},V_{T+1:T+\tau}),E_f^{'}))$

$\hat{Y}=\text{MLP}(\text{Decoder}(\text{Concat}(\Bar{A}\hat{X}_{T+1:T+\tau},V_{T+1:T+\tau}),E_f^{'}))$

\KwOut{Predicted future values $\hat{X}_{T+1:T+\tau}$, condition discriminator outputs $Y$ and $\hat{Y}$.}
\end{algorithm}

==> image/Parametric_analysi08.tex <==
\begin{figure*}[th]
    \begin{center}
	\parbox[t]{0.3\textwidth}{
		\includegraphics[width=0.3\textwidth]{image/lambda08.png}
		\label{fig:lambda}
	}
	\parbox[t]{0.3\textwidth}{
		\includegraphics[width=0.3\textwidth]{image/gamma08.png}
		\label{fig:gamma}
	}
	\parbox[t]{0.3\textwidth}{
		\includegraphics[width=0.3\textwidth]{image/beta08.png}
		\label{fig:beta}
	}	
	\caption{111}
	\end{center}
\end{figure*}

==> table/ablation.tex <==
\begin{table*}[t]
\begin{scriptsize}
\centering
\caption{Results of ablation experiments}
\begin{tabular}{lccc|ccc|ccc}
\hline
\toprule
 \multirow{&MAE &RMSE   &MAPE(\%) &MAE &RMSE   &MAPE(\%)&MAE &RMSE   &MAPE(\%)}
  &\multicolumn{}{c}{} 
&      &METR-LA     &  &      & PEMS-BAY     & &      & PEMS07     &            \\
\midrule
\hline
% ATP &2.54±0.03 &4.62±0.09 &6.28±0.018
% &1.12±0.01 &2.35±0.01 &2.36±0.01 &1.71±0.02 &3.11±0.05 &3.89±0.05\\
% w/o GANs &2.57±0.03 &4.62±0.10 &6.33±0.08 &1.12±0.01 &2.35±0.01 &2.36±0.01 &1.73±0.02 &3.12±0.05 &3.93±0.06\\
% w/o GCN&2.76±0.01 &5.19±0.01 &6.85±0.02 &1.15±0.01 &2.44±0.01 &2.43±0.01 &1.74±0.01  &3.19±0.01 &3.96±0.01\\
% w/o latent &2.73±0.02 &5.10±0.10 &6.81±0.03 &1.18±0.01 &2.49±0.01 &2.50±0.02 &1.80±0.02 &3.25±0.04 &4.09 ±0.05\\
% w/o transformer &2.59±0.01 &4.76±0.02 &6.43±0.02 &1.15±0.01 &2.38±0.02 &2.42±0.03 &1.79±0.02 &3.24±0.03 &4.11±0.05\\

ATP &2.54±0.03 &4.62±0.09 &6.28±0.018
&1.12±0.01 &2.35±0.01 &2.36±0.01 &1.84±0.01 &3.31±0.02 &4.18±0.03\\
w/o GANs &2.57±0.03 &4.62±0.10 &6.33±0.08 &1.12±0.01 &2.35±0.01 &2.36±0.01 &1.85±0.01 &3.33±0.02 &4.20±0.03\\
w/o GCN&2.76±0.01 &5.19±0.01 &6.85±0.02 &1.15±0.01 &2.44±0.01 &2.43±0.01 &1.90±0.01 &3.46±0.02 &4.35±0.02\\
w/o AM &2.73±0.02 &5.10±0.10 &6.81±0.03 &1.18±0.01 &2.49±0.01 &2.50±0.02 &1.97±0.02 &3.58±0.07 &4.53±0.09\\
w/o AP &2.59±0.01 &4.76±0.02 &6.43±0.02 &1.15±0.01 &2.38±0.02 &2.42±0.03 & 1.88±0.04 &3.42±0.09 &4.29±0.09 \\
\midrule
\hline
\multicolumn{}{c}{} 

&      &PEMS03     &  &      & PEMS04     & &      & PEMS08     &            \\
\midrule
\hline
% ATP	&13.12±0.09 &20.31±0.11 &16.15±0.06 &18.51±0.10 &29.70±0.16 &11.80±0.07 &14.24±0.06 &22.10±0.08 &10.42±0.04\\
% w/o GANs &13.13±0.09 &20.31±0.13 &16.18±0.06 &18.66±0.12 &29.56±0.12 &11.84±0.08 &14.30±0.06 &22.10±0.08 &10.46+0.04\\
% w/o GCN &13.47±0.02 &20.73±0.03 &16.68±0.01 &18.79±0.07 &30.04±0.10 &11.97±0.02 &14.50±0.07 &22.49±0.11 &10.58±0.03\\
% w/o latent &13.59±0.12 &20.81±0.15 &16.99±0.35&18.78±0.07 &30.12±0.16 &12.02±0.10 & 14.96±0.18 &22.99±0.22 &10.78±0.09\\
% w/o transformer &13.29±0.08 &20.56±0.08 &16.49±0.11 &18.71±0.17 &29.91±0.31 &11.92±0.12 &14.83±0.28 &22.79±0.34 &10.65±0.12 \\
ATP	&14.21±0.09 &22.08±0.11 &14.19±0.06 &19.77±0.10 &31.55±0.27 &12.48±0.10
&14.76±0.01 &23.17±0.02 &8.98±0.02\\
w/o GANs &14.22±0.09 &22.08±0.13 &14.22±0.06 &19.81±0.11 &31.60±0.27 &12.52±0.10 &14.80±0.08 &23.25±0.15 &8.99±0.08\\
w/o GCN &14.56±0.02 &22.50±0.03 &14.72±0.01  &19.98±0.10 &31.76±0.27 &12.66±0.09 &15.01±0.02 &23.64±0.04 &9.24 ±0.03\\
w/o AM &14.68±0.12 &22.58±0.15 &15.03±0.35  &19.97±0.11 &31.63±0.28 &12.63±0.11 &15.15±0.05 &23.72±0.12 &9.33 ±0.05\\
w/o AP &14.38±0.08 &22.33±0.08 &14.53±0.11  &19.90±0.13 &31.62±0.28 &12.61±0.12 &15.05±0.08 &23.54±0.14  &9.14 ±0.06\\
\midrule
\hline
\multicolumn{}{c}{} 

&      &Solar     &  &      & Electricity     & &      & ECG     &            \\
\midrule
\hline。
ATP &0.0458±0.0006 &0.1190±0.0009 &16.56±0.26 &0.0298±0.0005 & 0.0489±0.0013 &13.44±0.12 &0.0498±0.0003 &0.0743±0.0007 &10.25±0.14\\
w/o GANs 	&0.0458±0.0005 &0.1192±0.0006 &16.57±0.23 &0.0300±0.0004 &0.0490±0.0013 &13.53±0.12 &0.0500±0.0002 &0.0746±0.0004 &10.31±0.10\\
w/0 GCN&0.0496±0.0004 &0.1252±0.0008 &17.41±0.17 &0.0303±0.0001 &0.0506±0.0002 &13.58±0.07 &0.0501±0.0002 &0.0748±0.0004 &10.33±0.06\\
w/o AM &0.0471±0.0007 &0.1191±0.0006 &16.84±0.27 &0.0316±0.0004 &0.0515±0.0006 
&14.16±0.21 &0.0514±0.0005 &0.0763±0.0008 &10.70±0.10\\
w/o AP &0.0490±0.0006 &0.1236±0.0005 &17.67±0.19 &0.0320±0.0005 &0.0522±0.0012 &14.21±0.23 &0.0505±0.0001 &0.0749±0.0005 &10.46±0.04\\

\hline
\bottomrule
\end{tabular}
\label{tab:ablation}
\end{scriptsize}
\end{table*}

==> table/experiments.tex <==
\begin{table*}[t]
% \begin{scriptsize}
\centering
\caption{ Results of all methods for nine datasets}
\renewcommand\arraystretch{0.97}
\begin{tabular}{lccc|ccc|ccc}
\toprule
\hline
 \multirow{&MAE &RMSE   &MAPE(\%) &MAE &RMSE   &MAPE(\%)&MAE &RMSE   &MAPE(\%)}
  &\multicolumn{}{c}{} 
&      &METR-LA     &  &      & PEMS-BAY  & &      & PEMS07     &            
     \\
\midrule
\hline
ARIMA &3.43 &8.92 &8.12 &1.50 & 3.33 &3.10 &2.25 &4.29 &5.08\\
FC-LSTM   &3.44 &6.3 &9.6 &2.05 &4.19 &4.8 &3.57 &6.2 &8.6   \\
SFM &3.21 &6.2 &8.7 &2.03 &4.09 &4.4 &2.75 &4.32 &6.6 \\
N-BEATS &3.15 &6.12 &7.5 &1.75 &4.03 &4.1 &3.41 &5.52 &7.65 \\
DCRNN &2.77 &5.38 &7.3 &1.38 &2.95 &2.9 &2.25 &4.04 &5.30 \\
LSTNet &3.03 &5.91 &7.67 &1.86 &3.91 &3.1 &2.34 &4.26 &5.41 \\
ST-GCN &2.88 &5.74 &7.6 &1.36 &2.96 &2.9 &2.25 &4.04 &5.26 \\
TCN &2.74 &5.68 &6.54 &1.45 &3.01 &3.03 &3.25 &5.51 &6.7 \\
DeepState &2.72  &5.24 &6.8 &1.88 &3.04 &2.8 &3.95 &6.49 &7.9 \\
GraphWaveNet &2.69 &5.15 &6.9 &1.3 &2.74 &2.7 &- &- &- \\
DeepGLO &2.91 &5.48 &6.75 &1.39 &2.91 &3.01 &3.01 &5.25 &6.2 \\
StemGNN &2.56 &5.06 &6.46 &1.23 &2.48 &2.63  &2.14  &4.01  &5.01 \\
% TLAE &4.41 &8.70 &10.44 &2.43 &4.86 &5.63 &3.16 &5.69 &7.7329\\
AST &2.62 &5.21 &6.78 &1.23 &2.72 &2.46 &1.86  &3.53 &4.18\\
ATP &\textbf{2.54±0.03} &\textbf{4.62±0.09} &\textbf{6.28±0.018} &\textbf{1.12±0.01} &\textbf{2.35±0.01} &\textbf{2.36±0.01} &\textbf{1.84±0.01} &\textbf{3.31±0.02} &\textbf{4.18±0.03}\\
\midrule
\hline
\multicolumn{}{c}{} 

&      &PEMS03     &  &      & PEMS04     & &      & PEMS08     &            
 \\
\midrule
\hline
ARIMA &16.67 &25.61&16.30 &21.78 &34.21 &14.21 &17.70 &27.53 &10.80\\
FC-LSTM &21.33 &35.11 &23.33 &27.14 &41.59 &18.2 &22.2 &34.06 &14.2\\
SFM &17.67 &30.01 &18.33 &24.36 &37.10 &17.2 &16.01 &27.41 &10.4\\
N-BEATS &18.45 &31.23 &18.35 &25.56 &39.9 &17.18 &19.48 &28.32 &13.5\\
DCRNN &18.18 &30.31 &18.91 &24.7 &38.12 &17.12 &17.86 &27.83 &11.45\\
LSTNet &19.07 &29.67 &17.73 &24.04 &37.38 &17.01 &20.26 &31.96 &11.3\\
ST-GCN &17.49 &30.12 &17.15 &22.70 &35.50 &14.59 &18.02 &27.83 &11.4\\
TCN &18.23 &25.04 &19.44 &26.31 &36.11 &15.62 &15.93 &25.69 &16.5\\
DeepState &15.59 &\textbf{20.21} &18.69 &26.5 &33.0 &15.4 &19.34 &27.18 &16\\
GraphWaveNet &19.85 &32.94 &19.31 &26.85 &39.7 &17.29 &19.13 &28.16 &12.68\\
DeepGLO &17.25 &23.25 &19.27 &25.45 &35.9 &12.2 &15.12 &25.22 &13.2\\
StemGNN &14.32 &21.64 &16.24 &20.24 &32.15 &\textbf{10.03} &15.83 &24.93 &9.26\\
% TLAE &17.38 &31.03 &16.82 &22.11 &37.53 &14.38 &18.04 &28.24 &11.20\\
AST &14.44 &22.50 &14.90 &19.88 &31.83 &12.63
&15.32 &23.97 &9.32\\
ATP	&\textbf{14.21±0.09} &22.08±0.11 &\textbf{14.19±0.06} &\textbf{19.77±0.11} &\textbf{31.55±0.27} &12.48±0.10
&\textbf{14.76±0.01} &\textbf{23.17±0.02} &\textbf{8.98±0.02}\\
\midrule
\hline
\multicolumn{}{c}{} 

&      &Solar     &  &      & Electricity    & &      & ECG     &            
       \\
\midrule

% ARIMA &0.09 &0.15 &47.44 &0.078 &0.12 &24.96 &0.05 &0.08 &11.46\\
% FC-LSTM &0.13 &0.19 &27.01 &0.62 &0.2 &24.39 &0.32 &0.54 &31.0\\
% SFM &0.05 &0.09 &13.4 &0.08 &0.13 &17.3 &0.17 &0.58 &11.9\\
% N-BEATS &0.09 &0.15 &23.53 &- &- &- &0.08 &0.16 &12.428\\
% LSTNet &0.07 &0.19 &19.13 &0.06 &0.07 &14.97 &0.08 &0.12 &12.74\\
% TCN &0.06 &0.06 &21.1 &0.072 &0.51 &16.44 &0.1 &0.3 &19.03\\
% DeepState &0.06 &0.25 &19.4 &0.065 &0.67 &15.13 &0.09 &0.76 &19.21\\
% GraphWaveNet &0.05 &0.09 &18.12 &0.071 &0.53 &16.49 &0.19 &0.86 &19.67\\
% DeepGLO &0.09 &0.14 &21.6 &0.08 &0.14 &15.02 &0.09 &0.15 &12.45\\
% StemGNN &\textbf{0.03} &0.07 &11.55 &0.04 &0.06 &14.77 &0.05 &0.07 &10.58\\
\hline
ARIMA &0.0766 &0.1911 &25.17 &0.0755 &0.1152 &24.47  &0.0532 &0.0797 &10.73\\
FC-LSTM &0.1250 &0.2291 &27.01 &0.6192 &0.2004 &24.44 &0.2809 &0.3254 &31.02\\
SFM &0.0491 &0.1358 &19.45 &0.0856 &0.1298 &17.35 &0.1663 &0.2958 &11.92\\
N-BEATS &0.0855 &0.1897 &23.53 &- &- &- &0.0824 &0.1699 &12.43\\
LSTNet &0.0653 &0.2302 &19.13 &0.0611 &0.0752 &14.97 &0.0861 &0.1250 &12.74\\
TCN &0.0775 &0.1712 &24.79 & 0.0529 &0.0784 &18.20 &0.0506  & 0.0774 &10.32\\
DeepState &0.0610 &0.1901 &19.42 &0.0654 &0.3267 &15.13 &0.0832 &0.1976 &19.21\\
GraphWaveNet &0.0522 &0.1520 &18.12 &0.0712 &0.2917 &16.49 &0.0505 &0.0770 &10.91\\
DeepGLO &0.0925 &0.1532 &21.58 &0.0767 &0.1412 &15.02 &0.0672 &0.1534 &12.48\\
StemGNN &0.0483 &0.1259 &17.49 &0.0304 &\textbf{0.0479} &16.47 &0.0514 &0.0769 &10.83\\
% TLAE &0.0735 &0.1667 &24.86 &0.0526 &0.0805 &18.5944, &0.0511 &0.0786 &10.27 \\
%0.04894793649627764 0.07541389799746727 tensor(9.9088
AST &0.0555 &0.1453 &19.65 &0.0301 &0.0495 &15.57 &0.0515 &0.0774 &14.97
\\
ATP &\textbf{0.0458±0.0006} &\textbf{0.1190±0.0009} &\textbf{16.56±0.26} &\textbf{0.0299±0.0005} &0.0490±0.0011 &\textbf{13.49±0.17} &\textbf{0.0498±0.0003} &\textbf{0.0743±0.0007}&\textbf{10.25±0.14}\\
\hline
\bottomrule
\end{tabular}
\label{tab:experiments}
% \end{scriptsize}
\end{table*}

==> table/tau_07.tex <==
\begin{table}[t]
% \setlength\tabcolsep{3pt}  
\renewcommand\arraystretch{1.3}
% \tabcolsep=0.05cm
\centering
    \caption{Results of some methods at different $\tau$ under the dataset PEMS07.}
\begin{tabular}{l|cccc}
\toprule
\quad\tau  &3 &6  &9   \\
\midrule
StemGNN &2.144/4.01/5.01 &2.99/5.35/7.25 &3.16/6.34/8.43 \\
AST &1.97/3.63/4.41 &2.54/4.95/5.81 &3.03/6.01/7.05\\
Pyraformer &2.03/3.72/4.58 &2.61/4.93/6.98 &3.02/5.78/7.24 \\
ATP &\textbf{1.82}/\textbf{3.29}/\textbf{4.15} &\textbf{2.44}/\textbf{4.55}/\textbf{5.79}  &\textbf{2.93}/\textbf{5.41}/\textbf{6.98}\\

\bottomrule
\end{tabular}
\label{tab:tau_07}
\end{table}

==> table/tau_08.tex <==
\begin{table*}[t]
% \setlength\tabcolsep{3pt}  
\renewcommand\arraystretch{1.3}
% \tabcolsep=0.05cm
\centering
    \caption{Results of some methods at different $\tau$ under the dataset PEMS08}
\begin{tabular}{l|cccc}
\toprule
\quad\tau  &3 &6  &9  & 12   \\
\midrule
AST &15.32/23.97/9.32 &17.29/27.38/10.32 & &21.13/33.86/12.37\\
Pyraformer &15.39/23.97/9.66 &16.91/26.61/10.61 &18.20/28.89/11.35 &19.61/31.08/12.20 \\
ATP &14.73/23.09/8.91 &16.25/25.87/9.76 &17.65/28.33/10.54 &19.36/31.21/11.52 \\

\bottomrule
\end{tabular}
\label{tab:tau_08}
\end{table*}

==> table/web_traffic.tex <==
\begin{table}[t]
% \begin{scriptsize}
\centering
\caption{Results of the Wikipedia dataset}
\renewcommand\arraystretch{1.2}
\tabcolsep=0.1cm
% \begin{tabular}{l|ccc|ccc|ccc}
% \hline
% \toprule
% $\tau$ &      &7     &  &      & 14     & &      & 21     &            \\
% \hline
% Metrics &MAE &RMSE   &MAPE(\%) &MAE &RMSE   &MAPE(\%)&MAE &RMSE   &MAPE(\%)
%      \\
% \midrule
% StemGNN &0.0262 &0.0705 &69.02 &0.0270 &0.0674 &74.86 &0.0297 &0.0747 &83.73 \\
% AST &0.0267 &0.0747 &47.05 &0.0267 &0.0715 &53.49 &0.0301 &0.0799 &55.30\\
% Pyraformer &0.0304 &0.0715 &115.10 &0.0447 &0.0775 &191.92 &0.0368 &0.0795 &112.79\\
% ATP &0.0256 &0.0695 &42.84 &0.0264 &0.0664 &52.33 & 0.0286 &0.0736 &53.14 \\
% \midrule

% % \hline
% % \bottomrule
% \end{tabular}
\begin{tabular}{l|cc|cc|cc}
\hline
\toprule
$\tau$ &\multicolumn{2}{c|}{7 days}       &\multicolumn{2}{c|}{14 days}       & \multicolumn{2}{c}{21 days}              \\
\hline
Metrics &MAE &RMSE    &MAE &RMSE   &MAE &RMSE   
     \\
\midrule
StemGNN &0.0262 &0.0705  &0.0270 &0.0674  &0.0297 &0.0747  \\
AST &0.0267 &0.0747 &0.0267 &0.0715  &0.0301 &0.0799 \\
Pyraformer &0.0304 &0.0715  &0.0362 &0.0748  &0.0340 &0.0775 \\
ATP &\textbf{0.0256} &\textbf{0.0695}  &\textbf{0.0264} &\textbf{0.0664}  & \textbf{0.0286} &\textbf{0.0736}  \\
\midrule

\hline
% \bottomrule
\end{tabular}
\label{tab:web_traffic}
% \end{scriptsize}
\end{table}
